The Conformal Bootstrap: Theory, Numerical Techniques, and Applications

Conformal field theories have been long known to describe the fascinating universal physics of scale invariant critical points. They describe continuous phase transitions in fluids, magnets, and numerous other materials, while at the same time sit at the heart of our modern understanding of quantum field theory. For decades it has been a dream to study these intricate strongly coupled theories nonperturbatively using symmetries and other consistency conditions. This idea, called the conformal bootstrap, saw some successes in two dimensions but it is only in the last ten years that it has been fully realized in three, four, and other dimensions of interest. This renaissance has been possible both due to significant analytical progress in understanding how to set up the bootstrap equations and the development of numerical techniques for finding or constraining their solutions. These developments have led to a number of groundbreaking results, including world record determinations of critical exponents and correlation function coefficients in the Ising and $O(N)$ models in three dimensions. This article will review these exciting developments for newcomers to the bootstrap, giving an introduction to conformal field theories and the theory of conformal blocks, describing numerical techniques for the bootstrap based on convex optimization, and summarizing in detail their applications to fixed points in three and four dimensions with no or minimal supersymmetry.

==> theory/coordinates.tex <==
%!TEX root = ../Bootstrap-rmp.tex

\label{sec:conformal_frame}
 
Given a set of $n$ points, we can make use of conformal transformations to arrange them in convenient configurations. As an example, three points can be set to $y_{1,2,3}=0,\vec{e},\infty$, where $\vec{e}$ is any unit vector.\footnote{Formally $\infty$ can be though as the $L \vec{e}$, with $L\rightarrow\infty$} In doing so, we haven't exhausted the full symmetry: a residual $SO(d-1)$  remains. This symmetry can be though as the stabilizer group of the points $y_i$. If there are more than three points the stabilizer group of this configuration is instead $SO(d+2-m)$, where $m=\text{Min}(n,d+2)$. 

Notice that when $n>m$, there is no residual symmetry, and there are $(n-m)$ $d$-dimensional points that are completely unconstrained. The first $m$ points additionally contain $m(m-3)/2$ degrees of freedom. The unconstrained degrees of freedom can be identified with the number of independent conformally invariant cross-ratios that can be built out of $n$ points. 

The case we are primarily interested in is $n=4$. In this case the number of conformal invariants is always 2, except in $d=1$ which has only one invariant. These invariants can be identified with the cross ratios:
%
\begin{eqnarray}
\label{eq:uv}
u=\frac{x_{12}^2 x_{34}^2}{x_{13}^2 x_{24}^2}\,, \qquad v=\frac{x_{14}^2 x_{23}^2}{x_{13}^2 x_{24}^2}\,.
\end{eqnarray}

To make contact with the configuration above, in Euclidean signature we can introduce the convenient parametrization:
 \begin{eqnarray}
 \label{eq:conformalframe}
 &&x_1 = (0,0,\vec{0})\,,\nonumber\\
 &&x_2 = (0,1,\vec{0})\,,\nonumber\\
 &&x_3 = (\frac{z-\bar{z}}{2i},\frac{z+\bar{z}}{2},\vec{0})\,,\\
 &&x_4 = (0,\infty,\vec{0})\,,\nonumber
\end{eqnarray}
where $\vec{0}$ is a $(d-2)$-vector. Here $z,\bar{z}$ are complex conjugate variables. In Minkowski signature they become real and independent. With the above choice we then have the simple relations:
 \begin{eqnarray}
u= z\bar{z} \,, \qquad v= (1-z)(1-\bar{z})
\end{eqnarray}

A given choice of points $y_i$, as in Eq.~(\ref{eq:conformalframe}), is called a conformal frame. It can be thought of as a gauge fixing of most of the conformal symmetry. Because any coordinate configuration can be reduced to a given conformal frame and vice-versa, the knowledge of a correlation function in the conformal frame is sufficient to reconstruct it at any generic point through its covariant properties. This means that in order to classify the independent tensor structures or to impose consistency conditions (such as crossing), we can restrict to a conformal frame instead of working at generic coordinate configurations. Also, covariance with respect to the conformal group implies invariance under the stabilizer group~\cite{Kravchuk:2016qvl} . 

\begin{figure}[h!]
\begin{centering}
\includegraphics[width=0.6\columnwidth]{theory/radial.pdf}
\caption{\label{fig:radial}
Configuration defining radial coordinates in Eq.~(\ref{eq:reta}).
}
\end{centering}
\end{figure}

An alternative conformal frame, usually referred to as radial coordinates, was introduced in~\cite{Hogervorst:2013sma}. This corresponsd to setting the points $x_1,..,x_4$ as in Fig.~\ref{fig:radial}. The location of the points is parametrized in terms of  a  complex coordinate:
\begin{eqnarray}
\label{eq:reta}
&&\rho \equiv r e^{i \theta}\,, \qquad \eta = \cos \theta\,.
\end{eqnarray}
It is trivial to check that $r$ and $\eta$ are related to the usual cross ratios as:
\begin{eqnarray}
u=\frac{16 r^2}{\left(1+2 \eta  r+r^2\right)^2} \,, \nonumber\\
v= \frac{\left(1-2 \eta  r+r^2\right)^2}{\left(1+2 \eta  r+r^2\right)^2} \,.
\end{eqnarray}
In Euclidean signature, the relation with the complex $z$ ($\bar{z}=z^*$) is:
\begin{eqnarray}
\rho = \frac{z}{(1-\sqrt{1-z^2})^2} \,,
\qquad 
z = \frac{4\rho}{(1+\rho)^2}\,.\nonumber
\end{eqnarray}
As we will see in Sec.~\ref{sec:cb}, radial coordinates are very convenient for describing expansions of 4pt functions.









